The effects of rotation on the lithium depletion of G- and K-dwarfs in Messier 35

New fibre spectroscopy and radial velocities from the WIYN telescope are used to measure photospheric lithium in 242 high-probability, zero-age-main-sequence (ZAMS) F- to K-type members of the rich cluster M35. Combining these with published rotation periods, the connection between lithium depletion and rotation is studied in unprecedented detail. At $T_{\rm eff}<5500$ K there is a strong relationship between faster rotation and less Li depletion, although with a dispersion larger than measurement uncertainties. Components of photometrically identified binary systems follow the same relationship. A correlation is also established between faster rotation rate (or smaller Rossby number), decreased Li depletion and larger stellar radius at a given $T_{\rm eff}$. These results support models where starspots and interior magnetic fields lead to inflated radii and reduced Li depletion during the pre main sequence (PMS) phase for the fastest rotators. However, the data are also consistent with the idea that all stars suffered lower levels of Li depletion than predicted by standard PMS models, perhaps because of deficiencies in those models or because saturated levels of magnetic activity suppress Li depletion equally in PMS stars of similar $T_{\rm eff}$ regardless of rotation rate, and that slower rotators subsequently experience more mixing and post-PMS Li depletion.

==> latex_macros.tex <==
%
\newcommand{\rmsub}[2]{#1_{\rm #2}} 
\newcommand{\alfven}{Alfv\'en}
%
% USEFUL IN-TEXT CONTRACTIONS
%
\newcommand{\aat}{\mbox{\em AAT}}
\newcommand{\eso}{\mbox{\em ESO}}
\newcommand{\iue}{\mbox{\em IUE}}
\newcommand{\exosat}{\mbox{\em EXOSAT}}
\newcommand{\einstein}{\mbox{\em Einstein}}
\newcommand{\ginga}{\mbox{\em GINGA}}
\newcommand{\rosat}{\mbox{\em ROSAT}}
\newcommand{\caspec}{\mbox{\em CASPEC}}
\newcommand{\ucles}{\mbox{\em UCLES}}
\newcommand{\starlink}{\mbox{\em Starlink}}
\newcommand{\etal}{\mbox{\em et\ al.\ }}
\newcommand{\dex}[1]{\hbox{$\times\hbox{10}^{#1}$}}
\newcommand{\eex}[1]{\hbox{$\hbox{10}^{#1}$}}
\newcommand{\gpar}{\mbox{$g_{\parallel}$}}
\newcommand{\vsi}{\mbox{$v_e\,\sin\,i$}}
\newcommand{\vsini}{\mbox{$v_e\,\sin\,i$}}
\newcommand{\pattcit}[1]{\hbox{$^{(#1)}$}}
\newcommand{\pattcite}[1]{\hbox{$^{(#1)}$}}
%
% NAMES OF SPECTRAL LINES
%
\newcommand{\ha}{H$\alpha$}
\newcommand{\hb}{H$\beta$}
\newcommand{\hgam}{H$\gamma$}
\newcommand{\hdel}{H$\delta$}
\newcommand{\heps}{H$\epsilon$}
\newcommand{\lya}{\hbox{$\hbox{Ly}\alpha$}}
\newcommand{\naid}{\mbox{Na{\footnotesize I} {\sl D}}}
\newcommand{\caii}{Ca\,{\footnotesize II}}
\newcommand{\caiih}{Ca\,{\footnotesize II}~H}
\newcommand{\caiik}{Ca\,{\footnotesize II}~K}
\newcommand{\caiihk}{Ca\,{\footnotesize II}~H \&~K}
\newcommand{\mgii}{Mg\,{\footnotesize II}}
\newcommand{\mgiih}{\mbox{Mg{\footnotesize II} {\sl h}}}
\newcommand{\mgiik}{\mbox{Mg{\footnotesize II} {\sl k}}}
\newcommand{\mgiihk}{\mbox{Mg{\footnotesize II} {\sl h} \&\ {\sl k}}}
\newcommand{\lii}{Li\,{\footnotesize I}}
\newcommand{\fei}{Fe\,{\footnotesize I}}
\newcommand{\baii}{Ba\,{\footnotesize II}}
\newcommand{\ki}{K\,{\footnotesize I}}
\newcommand{\cai}{Ca\,{\footnotesize I}}
%
% UNITS
%
\newcommand{\ang}{\,\mbox{\AA}}
\newcommand{\Ang}{\ang}
\newcommand{\angstrom}{\ang}
\newcommand{\angstroms}{\ang}
\newcommand{\Angstrom}{\ang}
\newcommand{\Angstroms}{\ang}
\newcommand{\km}{\,km}
\newcommand{\Mpc}{\,\mbox{Mpc}}
\newcommand{\kpc}{\,\mbox{kpc}}
\newcommand{\kms}{\,km\,s$^{-1}$}
\newcommand{\ergs}{\,\mbox{$\mbox{erg}\,\mbox{s}^{-1}$}}
\newcommand{\ergsqcmsecang}{\,erg\,cm$^{-2}$\,s$^{-1}$\,\AA$^{-1}$}
\newcommand{\ergsqcm}{\,erg\,cm$^{-2}$}
\newcommand{\ergsqcmsec}{\,erg\,cm$^{-2}$\,s$^{-1}$}
\newcommand{\sqcm}{\,\mbox{$\mbox{cm}^{2}$}}
\newcommand{\cucm}{\,\mbox{$\mbox{cm}^{3}$}}
\newcommand{\persqcm}{\,\mbox{$\mbox{cm}^{-2}$}}
\newcommand{\gpersqcm}{\,\mbox{g}\persqcm}
\newcommand{\percc}{\,\mbox{$\mbox{cm}^{-3}$}}
\newcommand{\kev}{\,\mbox{keV}}
\newcommand{\kelvin}{\,K}
\newcommand{\kgmcube}{\,\mbox{$\mbox{kg}\,\mbox{m}^{-3}$}}
\newcommand{\dynsqcm}{\,\mbox{$\mbox{dyn}\,\mbox{cm}^{-2}$}}
\newcommand{\degrees}{\mbox{$^\circ$}}
\newcommand{\rstar}{\,\mbox{$\mbox{R}_*$}}
\newcommand{\mstar}{\,\mbox{$\mbox{M}_*$}}
\newcommand{\lstar}{\,\mbox{$\mbox{L}_*$}}
\newcommand{\vstar}{\,\mbox{$\mbox{V}_*$}}
\newcommand{\msun}{\,\mbox{$\mbox{M}_{\odot}$}}
\newcommand{\rsun}{\,\mbox{$\mbox{R}_{\odot}$}}
\newcommand{\lsun}{\,\mbox{$\mbox{L}_{\odot}$}}
\newcommand{\lx}{\,\mbox{$L_{\rm x}$}}
%
% REFERENCES
%
\newcommand{\reference}[5]{\noindent #1, #2. {\sl #3\/}, {\bf #4,} \,\mbox{#5}} 
\newcommand{\refnum}[4]{\noindent #1, #2. {\sl #3\/}, {\bf #4}}
\newcommand{\refbook}[3]{\noindent #1, #2. {\sl #3\/}}
\newcommand{\refpress}[3]{\noindent #1, #2. {\sl #3\/}, in press}
\newcommand{\refsub}[3]{\noindent #1, #2. {\sl #3\/}, submitted}
\newcommand{\refprep}[2]{\noindent #1, #2. In preparation}
%
% JOURNAL ABBREVIATIONS
%
\newcommand{\aanda}  {Astr.\ Astro\-phys.\nolinebreak\ }
\newcommand{\aasupp} {Astr.\ Astro\-phys.\nolinebreak\ Suppl.\nolinebreak\ }
\newcommand{\aj}     {Astron.\nolinebreak\ J.\nolinebreak\ }
\newcommand{\annrev} {Ann.\ Rev.\ Astr.\ Astro\-phys.\nolinebreak\ }
\newcommand{\acta}   {Acta Astron.\nolinebreak\ }
\newcommand{\apj}    {Astro\-phys.\nolinebreak\ J.\nolinebreak\ }
\newcommand{\apjs}   {Astro\-phys.\nolinebreak\ J.\ Suppl.\nolinebreak\ }
\newcommand{\apjsupp}{\apjs}
\newcommand{\aplett} {Astro\-phys.\nolinebreak\ Lett.\nolinebreak\ }
\newcommand{\gafd}   {Geo\-phys.~Astro\-phys.\ Fluid Dyn.\nolinebreak\ }
\newcommand{\ibvs}   {Inf.\ Bull.\ var.\ Stars\nolinebreak\ }
\newcommand{\jgr}    {J.\ Geo\-phys.~Res.\nolinebreak\ } 
\newcommand{\jpp}    {J.\ Plasma Phys.\nolinebreak\ }
\newcommand{\mn}     {Mon.\ Not.\ R.\ astr.\nolinebreak\ Soc.\nolinebreak\ }
\newcommand{\pf}     {Phys.\nolinebreak\ Fluids\nolinebreak\ }
\newcommand{\pasp}   {Publ.\ astr.\ Soc.\ Pacif.\nolinebreak\ }
\newcommand{\sovast} {Soviet astr.\nolinebreak\ }
\newcommand{\procasa}{Proc.\ Astr.\ Soc.\ Australia\nolinebreak\ }
\newcommand{\solp}   {Solar Phys.\nolinebreak\ }
\newcommand\mnras{MNRAS}
\newcommand\aap  {A\&A}
\newcommand\aaps  {A\&AS}

%
% MATH MACROS
%
\newcommand{\der}[1]{{\rm d}#1}
\newcommand{\deriv}[2]{\frac{{\rm d}#1}
                       {{\rm d}#2}} 
\newcommand{\sderiv}[2]{\frac{{\rm d}^2#1}\over
                       {{\rm d}#2^2}} 
\newcommand{\pderiv}[2]{\frac{\partial#1}
                       {\partial#2}} 
\newcommand{\spderiv}[2]{\frac{\partial^2#1}
                        {\partial#2^2}} 
\newcommand{\half}{\mbox{$\frac{1}{2}$}}
\newcommand{\twiddles}{\mbox{$\sim $}}
\newcommand{\varomega}{\varpi}
\newcommand{\twid}{\mbox{$\sim $}}
\newcommand{\bvec}[1]{\mbox{\boldmath ${#1}$}}
\newcommand{\uvec}[1]{\mbox{\boldmath $\hat{#1}$}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bd}{\begin{displaymath}}
\newcommand{\ed}{\end{displaymath}}
\newcommand{\del}{{\bf \nabla}}
\newcommand{\vhat}[1]{\mbox{$\bf \hat{#1}$}}













